Contextual Gradient Scaling for Few-Shot Learning

Model-agnostic meta-learning (MAML) is a well-known optimization-based meta-learning algorithm that works well in various computer vision tasks, e.g., few-shot classification. MAML is to learn an initialization so that a model can adapt to a new task in a few steps. However, since the gradient norm of a classifier (head) is much bigger than those of backbone layers, the model focuses on learning the decision boundary of the classifier with similar representations. Furthermore, gradient norms of high-level layers are small than those of the other layers. So, the backbone of MAML usually learns task-generic features, which results in deteriorated adaptation performance in the inner-loop. To resolve or mitigate this problem, we propose contextual gradient scaling (CxGrad), which scales gradient norms of the backbone to facilitate learning task-specific knowledge in the inner-loop. Since the scaling factors are generated from task-conditioned parameters, gradient norms of the backbone can be scaled in a task-wise fashion. Experimental results show that CxGrad effectively encourages the backbone to learn task-specific knowledge in the inner-loop and improves the performance of MAML up to a significant margin in both same- and cross-domain few-shot classification.

==> WACV 2022 CxGrad/materials/algorithm1_CxGrad.tex <==
\begin{algorithm}[t]
\fontsize{9}{11}\selectfont
\caption{Contextual Gradient Scaling (CxGrad)}

% https://tex.stackexchange.com/questions/200186/how-to-wrap-lines-correctly-inside-algorithmic
\makeatletter
\newcommand{\algmargin}{\the\ALG@thistlm}
\makeatother
\algnewcommand{\parState}[1]{\State%
  \parbox[t]{\dimexpr\linewidth-\algmargin}{\strut #1\strut}}

\textbf{Require: } $\alpha, \beta, \eta$: Learning rates\\
\textbf{Require: } $p(\mathcal{T})$: Distribution over tasks 

\begin{algorithmic}[1]
\State Randomly initialize $\boldtheta$ and $\boldphi$

\While{not done}
    %\State sample mini-batch of tasks $\task \sim p(\mathcal{T})$
    \State Sample a mini-batch of tasks $\{ \task \}_{i=1}^{B}$ from $p(\mathcal{T})$
    
    \For{$i \in [B]$}
    %\For{each task $\task$ in mini-batch}
        \State $\boldtheta_{i} \gets \boldtheta$
        \State Reset context parameters: $\boldnu_{i} = \bm{0}$
        \parState{%
            Sample support and query sets ($\support, \query$) from $\task$}
        \State $\boldtheta_{i}^{'} = $\texttt{IGS}($\boldtheta_{i}, \boldnu_{i}$)
        \State Compute $\nabla_{\boldnu_{i}} \mathcal{L}(\boldtheta_{i}^{'};\support)$ using support sets.
        \parState {%
            Update context parameters: \\
            $\boldnu_{i} \gets \boldnu_{i} - \beta \nabla_{\boldnu_{i}} \mathcal{L}(\boldtheta_{i}^{'};\support)$}
        
        \For {the number of inner-loop steps}
            \State $\boldtheta_{i} \gets $\texttt{IGS}($\boldtheta_{i}, \boldnu_{i}$)
            \parState {%
                Compute $\nabla_{(\boldtheta_{i}, \boldnu_{i})} \mathcal{L}(\boldtheta_{i};\support)$ using support sets.}
            \parState {%
                %Update network weights and context parameter:\\
                %$(\theta_{i}, \boldnu_{i}) \gets (\theta_{i}, \boldnu_{i}) - \alpha \nabla_{(\theta_{i}, \boldnu_{i})} \mathcal{L}(\theta_{i};\support)$}
                Update both network and context parameters:\\
                $\boldtheta_{i} \gets \boldtheta_{i} - \alpha \nabla_{\boldtheta_{i}} \mathcal{L}(\boldtheta_{i};\support)$\\
                $\boldnu_{i} \gets \boldnu_{i} - \beta \nabla_{\boldnu_{i}} \mathcal{L}(\boldtheta_{i};\support)$}
        \EndFor
    
    \State Compute $\mathcal{L}(\boldtheta_{i};\query)$ using query sets.
    \EndFor
    
    % \State $(\boldtheta, \boldphi) \gets (\boldtheta, \boldphi) - \eta \nabla_{(\boldtheta, \boldphi)}\sum_{i=1}^{B} \mathcal{L}(\boldtheta_{i};\query)$
    \parState {
        Update the model parameters: \\
        $(\boldtheta, \boldphi) \gets (\boldtheta, \boldphi) - \eta \nabla_{(\boldtheta, \boldphi)}\sum_{i=1}^{B} \mathcal{L}(\boldtheta_{i};\query)$
        }
    
\EndWhile

\end{algorithmic}
\label{alg:CxGrad}
\end{algorithm}

% \begin{algorithm}[t]
% \fontsize{9}{11}\selectfont
% \caption{Contextual Gradient Scaling (CxGrad)}

% % https://tex.stackexchange.com/questions/200186/how-to-wrap-lines-correctly-inside-algorithmic
% \makeatletter
% \newcommand{\algmargin}{\the\ALG@thistlm}
% \makeatother
% \algnewcommand{\parState}[1]{\State%
%   \parbox[t]{\dimexpr\linewidth-\algmargin}{\strut #1\strut}}

% \textbf{Require: } $\alpha, \beta, \eta$: Learning rates\\
% \textbf{Require: } $p(\mathcal{T})$: Distribution over tasks 

% \begin{algorithmic}[1]
% \State Randomly initialize $\theta$ and $\phi$

% \While{not done}
%     %\State sample mini-batch of tasks $\task \sim p(\mathcal{T})$
%     \State Sample a mini-batch of tasks $\{ \task \}_{i=1}^{B}$ from $p(\mathcal{T})$
    
%     \For{$i \in [B]$}
%     %\For{each task $\task$ in mini-batch}
%         \State $\theta_{i} \gets \theta$
%         \State Reset context parameters: $\boldnu_{i} = \bm{0}$
%         \parState{%
%             Sample support and query sets ($\support, \query$) from $\task$}
%         \State $\theta_{i}^{'} = $\texttt{IGS}($\theta_{i}, \boldnu_{i}$)
%         \State Compute $\nabla_{\boldnu_{i}} \mathcal{L}(\theta_{i}^{'};\support)$ using support sets.
%         \parState {%
%             Update context parameters: \\
%             $\boldnu_{i} \gets \boldnu_{i} - \beta \nabla_{\boldnu_{i}} \mathcal{L}(\theta_{i}^{'};\support)$}
        
%         \For {the number of inner-loop steps}
%             \State $\theta_{i} \gets $\texttt{IGS}($\theta_{i}, \boldnu_{i}$)
%             \parState {%
%                 Compute $\nabla_{(\theta_{i}, \boldnu_{i})} \mathcal{L}(\theta_{i};\support)$ using support sets.}
%             \parState {%
%                 %Update network weights and context parameter:\\
%                 %$(\theta_{i}, \boldnu_{i}) \gets (\theta_{i}, \boldnu_{i}) - \alpha \nabla_{(\theta_{i}, \boldnu_{i})} \mathcal{L}(\theta_{i};\support)$}
%                 Update both network and context parameters:\\
%                 $\theta_{i} \gets \theta_{i} - \alpha \nabla_{\theta_{i}} \mathcal{L}(\theta_{i};\support)$\\
%                 $\boldnu_{i} \gets \boldnu_{i} - \beta \nabla_{\boldnu_{i}} \mathcal{L}(\theta_{i};\support)$}
%         \EndFor
    
%     \State Compute $\mathcal{L}(\theta_{i};\query)$ using query sets.
%     \EndFor
    
%     \State $(\theta, \boldphi) \gets (\theta, \boldphi) - \eta \nabla_{(\theta, \boldphi)}\sum_{\task} \mathcal{L}(\theta_{i};\query)$
    
% \EndWhile

% \end{algorithmic}
% \label{alg:CxGrad}
% \end{algorithm}

==> WACV 2022 CxGrad/materials/algorithm2_IGS.tex <==
% \begin{algorithm}[t]
% \fontsize{9}{11}\selectfont
% \caption{Implicit Gradient Scaling (IGS)}

% % https://tex.stackexchange.com/questions/200186/how-to-wrap-lines-correctly-inside-algorithmic
% \makeatletter
% \newcommand{\algmargin}{\the\ALG@thistlm}
% \makeatother
% \algnewcommand{\parState}[1]{\State%
%   \parbox[t]{\dimexpr\linewidth-\algmargin}{\strut #1\strut}}

% \textbf{Input: } Model parameters $\boldtheta_{i}$, context vector $\boldnu_{i}$

% \begin{algorithmic}[1]

% \State $\{ \boldomega_{i}, \boldpsi_{i} \} \gets \boldtheta_{i}$
% \State $\{\gamma^{(\ell)}_{i}\}^L_{\ell=1} = g_{\boldphi}(\boldnu_{i})$
% \State $\boldomega_{i} \gets \bigg\{ \gamma^{(\ell)}_{i} \boldomega^{(\ell)}_{i} / \lVert \boldomega^{(\ell)}_{i} \rVert \bigg\}^{L}_{\ell=1}$
% \State $\boldtheta_{i} \gets \{ \boldomega_{i}, \boldpsi_{i} \}$
% \State \textbf{Return} $\boldtheta_{i}$

% \end{algorithmic}
% \label{alg:IGS}
% \end{algorithm}

\begin{algorithm}[t]
\fontsize{9}{11}\selectfont
\caption{Implicit Gradient Scaling (IGS)}

% https://tex.stackexchange.com/questions/200186/how-to-wrap-lines-correctly-inside-algorithmic
\makeatletter
\newcommand{\algmargin}{\the\ALG@thistlm}
\makeatother
\algnewcommand{\parState}[1]{\State%
  \parbox[t]{\dimexpr\linewidth-\algmargin}{\strut #1\strut}}

\textbf{Input: } Model parameters $\boldtheta_{i} = \{ \boldomega_{i}, \boldpsi_{i} \}$\\ \textbf{Input: } Context parameters $\boldnu_{i}$

\begin{algorithmic}[1]

%\State $\{ \boldomega_{i}, \boldpsi_{i} \} \gets \boldtheta_{i}$
\parState {% 
Generate a set of scaling factors: \\ $\{\gamma^{(\ell)}_{i}\}^L_{\ell=1} = g_{\boldphi}(\boldnu_{i})$}
\parState {% 
Scales the parameters of the backbone: \\ $\boldomega_{i} \gets \bigg\{ \gamma^{(\ell)}_{i} \boldomega^{(\ell)}_{i} / \lVert \boldomega^{(\ell)}_{i} \rVert \bigg\}^{L}_{\ell=1}$}
%\State $\boldtheta_{i} \gets \{ \boldomega_{i}, \boldpsi_{i} \}$
\State \textbf{Return} $\boldtheta_{i}$

\end{algorithmic}
\label{alg:IGS}
\end{algorithm}

==> WACV 2022 CxGrad/materials/figure1_main.tex <==
% \begin{figure}
% \begin{center}
%     \begin{subfigure}[t]{\linewidth}
%         \centering
%         \includegraphics[width=.75\linewidth]{materials/png/representation_maml.png}
%         \setlength{\abovecaptionskip}{2pt}
%         \setlength{\belowcaptionskip}{10pt}
%         \caption{MAML}
%     \end{subfigure}
%     \hspace{2em}
%     \begin{subfigure}[t]{\linewidth}
%         \centering
%         \includegraphics[width=.75\linewidth]{materials/png/representation_cxgrad.png}
%         \setlength{\abovecaptionskip}{2pt}
%         \setlength{\belowcaptionskip}{0pt}
%         \caption{CxGrad}
%     \end{subfigure}
% \end{center}
%     \setlength{\abovecaptionskip}{0pt}
%     %\setlength{\belowcaptionskip}{-5pt}
%     \caption{An overview of the adaptation scheme of MAML and CxGrad. Shapes represent samples belonging to different classes, and lines represent decision boundaries of the classifier. (a) MAML focuses on updating the decision boundary to adapt to a given task. However, (b) CxGrad mainly updates the feature extractor rather than the decision boundary. As a result, although training tasks and target tasks are far different, we can get optimized representation for the target tasks. Furthermore, CxGrad updates the decision boundary based on the changed representation.}
% \label{fig:concept}
% \end{figure}

\begin{figure}
\begin{center}
    \begin{subfigure}[t]{\linewidth}
        \centering
        \includegraphics[width=.9\linewidth]{materials/png/representation.png}
        \setlength{\abovecaptionskip}{2pt}
        \setlength{\belowcaptionskip}{10pt}
    \end{subfigure}
\end{center}
    \setlength{\abovecaptionskip}{0pt}
    %\setlength{\belowcaptionskip}{-5pt}
    \caption{An overview of the adaptation scheme of MAML and CxGrad. Shapes represent samples belonging to different classes, and lines represent decision boundaries of the classifier. MAML focuses on updating the decision boundary to adapt to a given task. However, CxGrad mainly updates the feature extractor rather than the decision boundary. As a result, although training tasks and target tasks are far different, we can get optimized representation for the target tasks. Furthermore, CxGrad updates the decision boundary based on the changed representation.}
\label{fig:concept}
\end{figure}

==> WACV 2022 CxGrad/materials/figure2_gradient_norm.tex <==
\begin{figure*}[ht]
\begin{center}
    \begin{subfigure}[t]{.45\linewidth}
        \centering
        \includegraphics[width=1\linewidth]{materials/png/gradient_norm_MAML.png}
        \caption{MAML}
        \label{fig:gradient_norm_MAML}
    \end{subfigure}
    % \begin{subfigure}[t]{.33\linewidth}
    %     \centering
    %     \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
    %     \caption{BOIL}
    %     \label{fig:gradient_norm_BOIL}
    % \end{subfigure}
    \begin{subfigure}[t]{.45\linewidth}
        \centering
        \includegraphics[width=1\linewidth]{materials/png/gradient_norm_CxGrad.png}
        \caption{CxGrad}
        \label{fig:gradient_norm_CxGrad}
    \end{subfigure}
\end{center}
    \setlength{\abovecaptionskip}{0pt}
    %\setlength{\belowcaptionskip}{-5pt}
    \caption{Gradient norms of MAML and CxGrad during adaptation in meta-training. Gradient norms are averaged over inner-loop steps and tasks of the batch. In (a) MAML, the gradient norm of the classifier is bigger than those of backbone layers. Furthermore, gradient norms of low- and mid-levels are bigger than those of high-level layers. Considering the fact that high-level layers learn more discriminative features, MAML reuses similar representation from meta-knowledge and heavily depends on updating a decision boundary. However, in (b) CxGrad, gradient norms of high-level layers are much bigger than the others. Also, the norm gets smaller near the front side of the backbone. As a result, CxGrad focuses on changing representation and the backbone learns to extract task-specific features.}
    %This matches the fact that higher level learns task-specific features, which implies representation change is an significant role of performance in optimization-based meta-learning.}
\label{fig:gradient_norm}
\end{figure*}

==> WACV 2022 CxGrad/materials/figure3_feature_similarity.tex <==
\begin{figure}[t]
\setlength{\abovecaptionskip}{0pt}
\setlength{\belowcaptionskip}{5pt}
\begin{center}
    \includegraphics[width=.8\linewidth]{materials/png/CKA_feature_similarity.png}
\end{center}
\caption{CKA values of three optimization-based meta-learning algorithms. The x-axis means each layer in the backbone and the y-axis means the CKA value.}
\label{fig:feature_sim}
\end{figure}

==> WACV 2022 CxGrad/materials/figure4_embedding.tex <==
\begin{figure*}[t]
\begin{center}
    \begin{subfigure}[t]{.48\linewidth}
        \centering
        \begin{subfigure}[t]{.49\linewidth}
            \includegraphics[width=\linewidth]{materials/png/MAML_0_miniImageNet_before.png}
        \end{subfigure}
        \begin{subfigure}[t]{.49\linewidth}
            \includegraphics[width=\linewidth]{materials/png/MAML_0_miniImageNet_after.png}
        \end{subfigure}
        %\caption{MAML}
    \end{subfigure}
    \hspace*{5mm}
    \begin{subfigure}[t]{.48\linewidth}
        \centering
        \begin{subfigure}[t]{.49\linewidth}
            \includegraphics[width=\linewidth]{materials/png/CxGrad_1_miniImageNet_before.png}
        \end{subfigure}
        \begin{subfigure}[t]{.49\linewidth}
            \includegraphics[width=\linewidth]{materials/png/CxGrad_1_miniImageNet_after.png}
        \end{subfigure}
        %\caption{CxGrad}
    \end{subfigure}
    \end{center}
    
\begin{center}
    \begin{subfigure}[t]{.48\linewidth}
        \centering
        \begin{subfigure}[t]{.49\linewidth}
            \includegraphics[width=\linewidth]{materials/png/MAML_1_CUB_before.png}
        \end{subfigure}
        \begin{subfigure}[t]{.49\linewidth}
            \includegraphics[width=\linewidth]{materials/png/MAML_1_CUB_after.png}
        \end{subfigure}
        \caption{MAML}
    \end{subfigure}
    \hspace*{5mm}
    \begin{subfigure}[t]{.48\linewidth}
        \centering
        \begin{subfigure}[t]{.49\linewidth}
            \includegraphics[width=\linewidth]{materials/png/CxGrad_2_CUB_before.png}
        \end{subfigure}
        \begin{subfigure}[t]{.49\linewidth}
            \includegraphics[width=\linewidth]{materials/png/CxGrad_2_CUB_after.png}
        \end{subfigure}
        \caption{CxGrad}
    \end{subfigure}
\end{center}
\setlength{\abovecaptionskip}{0pt}
%\setlength{\belowcaptionskip}{pt}
\caption{Visualization for latent feature representation using t-SNE. The first row is visualizations for meta-test on miniImageNet and the second row is on CUB. Each shape represents each class and the latent features are from the output of the last convolutional block of the backbone.}
\label{fig:embedding}
\end{figure*}

==> WACV 2022 CxGrad/materials/figure5_landscape.tex <==
\begin{figure*}[t]
\begin{center}
    \begin{subfigure}[t]{.33\linewidth}
        \centering
        \includegraphics[width=1\linewidth]{materials/png/loss_landscape.png}
        \caption{Loss landscape}
        \label{fig:landscape_loss}
    \end{subfigure}
    \begin{subfigure}[t]{.33\linewidth}
        \centering
        \includegraphics[width=1\linewidth]{materials/png/gradient_predictiveness.png}
        \caption{Gradient predictiveness}
        \label{fig:landscape_gradient}
    \end{subfigure}
    \begin{subfigure}[t]{.33\linewidth}
        \centering
        \includegraphics[width=1\linewidth]{materials/png/lipschitzness.png}
        \caption{``effective'' $\beta$ smoothness}
        \label{fig:landscape_beta}
    \end{subfigure}
\end{center}
    \setlength{\abovecaptionskip}{0pt}
    %\setlength{\belowcaptionskip}{pt}
   %\caption{Optimization landscape of various gradient-based meta-learning methods. In \cite{how_does_BN}, they analyze the smoothing effect of Batch Normalization. n \cite{L2F} the authors analyze the training stability in both inner-loop and outer-loop in terms of smoothness.}
   \caption{Optimization landscape during adaptation. Like other experiments, we plot these results from 5-way 5-shot miniImageNet few-shot classification. In order to analyze the landscape, we update the model parameter from a certain inner-loop step with various range of learning rates. We refer to these updated parameters as \textit{points}. With these, we can analyze the local landscape from the certain step. (a) We measure the variation in loss calculated at the \textit{points}. (b) We measure the variation in $\ell_{2}$ distance between the gradients at the certain step and at each \textit{point}. (c) ``effective'' $\beta$ smoothness refers to the maximum $\ell_{2}$ difference of (b) over distance as we move to the corresponding \textit{point} from the certain step.}
\label{fig:landscape}
\end{figure*}

==> WACV 2022 CxGrad/materials/table1_benchmark.tex <==
% \begin{table}
% \fontsize{8}{10}\selectfont
% \begin{center}
% \begin{tabular}{c|c|cc}
% \hline \hline
% \multirow{2}{*}{\textbf{Method}} \tstrut & \multirow{2}{*}{\textbf{Backbone}} \tstrut &
% \multicolumn{2}{c}{\textbf{miniImageNet}} \tstrut\bstrut\\
% & & 1-shot & 5-shot \bstrut \\
% \hline
% MatchingNet~\cite{MatchingNet} \tstrut & 4 conv & 43.44 $\pm$ 0.77\%          & 55.31 $\pm$ 0.73\% \\
% RelationNet~\cite{RelationNet}         & 4 conv & 50.44 $\pm$ 0.82\%          & 65.32 $\pm$ 0.70\% \\
% ProtoNet~\cite{ProtoNet}               & 4 conv & 49.42 $\pm$ 0.78\%          & 68.20 $\pm$ 0.66\% \\
% \hdashline
% MAML~\cite{MAML}                       & 4 conv & 48.70 $\pm$ 1.75\%          & 63.11 $\pm$ 0.91\% \\
% CAVIA (512)~\cite{CAVIA}               & 4 conv & 51.82 $\pm$ 0.65\%          & 65.85 $\pm$ 0.55\% \\
% BOIL~\cite{BOIL}                       & 4 conv & 49.61 $\pm$ 0.16\%          & 66.45 $\pm$ 0.37\% \\
% MAML++~\cite{MAML++}                   & 4 conv & 52.15 $\pm$ 0.26\%          & 68.32 $\pm$ 0.44\% \\
% ALFA~\cite{ALFA}                       & 4 conv & 50.58 $\pm$ 0.51\%          & 69.12 $\pm$ 0.47\% \\
% ModGrad~\cite{ModGrad}                 & 4 conv & \textbf{53.20 $\pm$ 0.86\%} & 69.17 $\pm$ 0.69\% \\
% L2F~\cite{L2F}                         & 4 conv & 52.10 $\pm$ 0.50\%          & 69.38 $\pm$ 0.46\% \\
% CxGrad (Ours) \bstrut                  & 4 conv & 51.80 $\pm$ 0.46\% & \textbf{69.91 $\pm$ 0.42\%} \\
% % \hline
% % MAML            & ResNet12 & 51.03 $\pm$ 0.50\% & 68.26 $\pm$ 0.47\% \\
% % BOIL            & ResNet12 & -                & 70.50 $\pm$ 0.28\% \\
% % L2F             & ResNet12 & 57.48 $\pm$ 0.49\% & 74.68 $\pm$ 0.43\% \\
% % CxGrad (Ours)   & - & - \\
% \hline
% \end{tabular}
% \end{center}
% \caption{Test accuracy on 5-way miniImageNet classification. Our method outperforms the others in 5-shot case and shows comparable result in 1-shot case.}
% \label{table:mini_imagenet}
% \end{table}

% \begin{table*}
% %\fontsize{8}{10}\selectfont
% \begin{center}
% \begin{tabular}{c|c|cc|cc}
% \hline \hline
% \multirow{2}{*}{\textbf{Method}} \tstrut & \multirow{2}{*}{\textbf{Backbone}} \tstrut &
% \multicolumn{2}{c|}{\textbf{miniImageNet}} & \multicolumn{2}{c}{\textbf{tieredImageNet}} \\
% & & 1-shot & 5-shot & 1-shot & 5-shot \\
% \hline
% MatchingNet~\cite{MatchingNet} \tstrut & 4 conv & 43.44 $\pm$ 0.77\%          & 55.31 $\pm$ 0.73\% & -- & --\\
% RelationNet~\cite{RelationNet}         & 4 conv & 50.44 $\pm$ 0.82\%          & 65.32 $\pm$ 0.70\% & -- & --\\
% ProtoNet~\cite{ProtoNet}               & 4 conv & 49.42 $\pm$ 0.78\%          & 68.20 $\pm$ 0.66\% & -- & --\\
% \hdashline
% MAML~\cite{MAML}                       & 4 conv & 48.70 $\pm$ 1.75\%          & 63.11 $\pm$ 0.91\% & 49.06 $\pm$ 0.50\% & 67.48 $\pm$ 0.47\%\\
% CAVIA (512)~\cite{CAVIA}               & 4 conv & 51.82 $\pm$ 0.65\%          & 65.85 $\pm$ 0.55\% & -- & --\\
% BOIL~\cite{BOIL}                       & 4 conv & 49.61 $\pm$ 0.16\%          & 66.45 $\pm$ 0.37\% & 48.58 $\pm$ 0.27\% & 69.37 $\pm$ 0.12\%\\
% MAML++~\cite{MAML++}                   & 4 conv & 52.15 $\pm$ 0.26\%          & 68.32 $\pm$ 0.44\% & -- & --\\
% ALFA~\cite{ALFA}                       & 4 conv & 50.58 $\pm$ 0.51\%          & 69.12 $\pm$ 0.47\% & 53.16 $\pm$ 0.49\% & 70.54 $\pm$ 0.46\%\\
% ModGrad~\cite{ModGrad}                 & 4 conv & \textbf{53.20 $\pm$ 0.86\%} & 69.17 $\pm$ 0.69\% & -- & --\\
% L2F~\cite{L2F}                         & 4 conv & 52.10 $\pm$ 0.50\%          & 69.38 $\pm$ 0.46\% & 54.40 $\pm$ 0.50\% & 73.34 $\pm$ 0.44\%\\
% CxGrad (Ours) \bstrut                  & 4 conv & 51.80 $\pm$ 0.46\% & \textbf{69.91 $\pm$ 0.42\%} & \textbf{55.55 $\pm$ 0.46\%} & \textbf{73.55 $\pm$ 0.41\%}\\
% % \hline
% % MAML            & ResNet12 & 51.03 $\pm$ 0.50\% & 68.26 $\pm$ 0.47\% \\
% % BOIL            & ResNet12 & -                & 70.50 $\pm$ 0.28\% \\
% % L2F             & ResNet12 & 57.48 $\pm$ 0.49\% & 74.68 $\pm$ 0.43\% \\
% % CxGrad (Ours)   & - & - \\
% \hline
% \end{tabular}
% \end{center}
% \caption{Test accuracy on 5-way miniImageNet classification. Our method outperforms the others in 5-shot case and shows comparable result in 1-shot case.}
% \label{table:mini_imagenet}
% \end{table*}

% \begin{table*}
% \begin{center}
% %\fontsize{8}{10}\selectfont
% %\begin{tabular}{c|c|c|c|c}
% \begin{tabularx}{\textwidth}{>{\centering\arraybackslash}X|>{\centering\arraybackslash}X|
% >{\centering\arraybackslash}X|>{\centering\arraybackslash}X|>{\centering\arraybackslash}X}
% \hline \hline
% \multirow{2}{*}{\textbf{Method}} \tstrut & \multicolumn{2}{c|}{\textbf{miniImageNet}} & \multicolumn{2}{c}{\textbf{tieredImageNet}} \bstrut \\
% \cline{2-5}
% \tstrut & \textbf{1-shot} & \textbf{5-shot} & \textbf{1-shot} & \textbf{5-shot} \bstrut \\
% %\tstrut & 1-shot & 5-shot & 1-shot & 5-shot \bstrut \\
% \hline
% MatchingNet~\cite{MatchingNet} \tstrut & $43.44 \pm 0.77\%$          & $55.31 \pm 0.73\%$ & -- & --\\
% RelationNet~\cite{RelationNet}         & $50.44 \pm 0.82\%$          & $65.32 \pm 0.70\%$ & -- & --\\
% ProtoNet~\cite{ProtoNet}               & $49.42 \pm 0.78\%$          & $68.20 \pm 0.66\%$ & -- & --\\
% %\hdashline
% MAML~\cite{MAML}                       & $48.70 \pm 1.75\%$          & $63.11 \pm 0.91\%$ & $49.06 \pm 0.50\%$ & $67.48 \pm 0.47\%$\\
% CAVIA (512)~\cite{CAVIA}               & $51.82 \pm 0.65\%$          & $65.85 \pm 0.55\%$ & -- & --\\
% BOIL~\cite{BOIL}                       & $49.61 \pm 0.16\%$          & $66.45 \pm 0.37\%$ & $48.58 \pm 0.27\%$ & $69.37 \pm 0.12\%$\\
% MAML++~\cite{MAML++}                   & $52.15 \pm 0.26\%$          & $68.32 \pm 0.44\%$ & -- & --\\
% ALFA~\cite{ALFA}                       & $50.58 \pm 0.51\%$          & $69.12 \pm 0.47\%$ & $53.16 \pm 0.49\%$ & $70.54 \pm 0.46\%$\\
% ModGrad~\cite{ModGrad}                 & \vcsb{53.20 \pm 0.86\%} & $69.17 \pm 0.69\%$ & -- & --\\
% L2F~\cite{L2F}                         & $52.10 \pm 0.50\%$          & $69.38 \pm 0.46\%$ & $54.40 \pm 0.50\%$ & $73.34 \pm 0.44\%$\\
% CxGrad (Ours) \bstrut                  & $51.80 \pm 0.46\%$ & \vcsb{69.82 \pm 0.42\%} & \vcsb{55.55 \pm 0.46\%} & \vcsb{73.55 \pm 0.41\%}\\
% % \hline
% % MAML            & ResNet12 & 51.03 $\pm$ 0.50\% & 68.26 $\pm$ 0.47\% \\
% % BOIL            & ResNet12 & -                & 70.50 $\pm$ 0.28\% \\
% % L2F             & ResNet12 & 57.48 $\pm$ 0.49\% & 74.68 $\pm$ 0.43\% \\
% % CxGrad (Ours)   & - & - \\
% \hline
% %\end{tabular}
% \end{tabularx}
% \end{center}
% \caption{Test accuracy on 5-way miniImageNet classification. Our method outperforms the others in 5-shot case and shows comparable result in 1-shot case.}
% \label{table:benchmark}
% \vspace{-2mm}
% \end{table*}

\begin{table*}
\setlength{\abovecaptionskip}{0pt}
%\setlength{\belowcaptionskip}{-5pt}
\begin{center}
%\fontsize{8}{10}\selectfont
%\begin{tabular}{c|c|c|c|c}
\begin{tabularx}{\textwidth}{>{\centering\arraybackslash}X>{\centering\arraybackslash}X
>{\centering\arraybackslash}X>{\centering\arraybackslash}X>{\centering\arraybackslash}X}
\toprule %\toprule
\multirow{2}{*}{\textbf{Method}} & \multicolumn{2}{c}{\textbf{miniImageNet}} & \multicolumn{2}{c}{\textbf{tieredImageNet}} \\
%\cmidrule{2-3} %\cmidrule{4-5}
& \textbf{1-shot} & \textbf{5-shot} & \textbf{1-shot} & \textbf{5-shot} \\
%\tstrut & 1-shot & 5-shot & 1-shot & 5-shot \bstrut \\
\midrule
MatchingNet~\cite{MatchingNet}         & $43.44 \pm 0.77\%$          & $55.31 \pm 0.73\%$      & --                  & --\\
RelationNet~\cite{RelationNet}         & $50.44 \pm 0.82\%$          & $65.32 \pm 0.70\%$      & --                  & --\\
ProtoNet~\cite{ProtoNet}               & $49.42 \pm 0.78\%$          & $68.20 \pm 0.66\%$      & --                  & --\\
%\hdashline
MAML~\cite{MAML}                       & $48.70 \pm 1.84\%$          & $63.11 \pm 0.92\%$      & $49.06 \pm 0.50\%$  & $67.48 \pm 0.47\%$\\
CAVIA (512)~\cite{CAVIA}               & $51.82 \pm 0.65\%$          & $65.85 \pm 0.55\%$      & --                  & --\\
BOIL~\cite{BOIL}                       & $49.61 \pm 0.16\%$          & $66.45 \pm 0.37\%$      & $48.58 \pm 0.27\%$  & $69.37 \pm 0.12\%$\\
MAML++~\cite{MAML++}                   & $52.15 \pm 0.26\%$          & $68.32 \pm 0.44\%$      & --                  & --\\
ALFA~\cite{ALFA}                       & $50.58 \pm 0.51\%$          & $69.12 \pm 0.47\%$      & $53.16 \pm 0.49\%$  & $70.54 \pm 0.46\%$\\
ModGrad~\cite{ModGrad}                 & \vcsb{53.20 \pm 0.86\%}     & $69.17 \pm 0.69\%$      & --                  & --\\
L2F~\cite{L2F}                         & $52.10 \pm 0.50\%$          & $69.38 \pm 0.46\%$      & $54.40 \pm 0.50\%$  & $73.34 \pm 0.44\%$\\
CxGrad (Ours)                          & $51.80 \pm 0.46\%$          & \vcsb{69.82\pm0.42\%} & \vcsb{55.55\pm0.46\%} & \vcsb{73.55\pm0.41\%}\\
% \hline
% MAML            & ResNet12 & 51.03 $\pm$ 0.50\% & 68.26 $\pm$ 0.47\% \\
% BOIL            & ResNet12 & -                & 70.50 $\pm$ 0.28\% \\
% L2F             & ResNet12 & 57.48 $\pm$ 0.49\% & 74.68 $\pm$ 0.43\% \\
% CxGrad (Ours)   & - & - \\
\bottomrule
%\end{tabular}
\end{tabularx}
\end{center}
\caption{Test accuracy on 5-way miniImageNet and tieredImageNet classification. CxGrad outperforms the others in 5-shot on both datasets and in 1-shot on tieredImageNet. CxGrad shows comparable result even in 1-shot on miniImageNet.}
\label{table:benchmark}
\end{table*}

==> WACV 2022 CxGrad/materials/table2_cross_domain.tex <==
% \begin{table*}[t]
% %\fontsize{7}{10}\selectfont
% \begin{center}
% %\begin{tabular}{c|c|c|c|c}
% \begin{tabularx}{\textwidth}{>{\centering\arraybackslash}X|>{\centering\arraybackslash}X|
% >{\centering\arraybackslash}X|>{\centering\arraybackslash}X}
% \hline \hline
% \multirow{2}{*}{\textbf{Method}} \tstrut & \multicolumn{3}{c}{\textbf{miniImageNet}} \bstrut\\
% \cline{2-4}
% & \textbf{$\to$ CUB} & \textbf{$\to$ FC100} & \textbf{$\to$ CIFAR-FS}\tstrut \bstrut\\
% %\tstrut & $\to$ CUB & $\to$ Omniglot & $\to$ FC100 & $\to$ CIFAR-FS \bstrut\\
% % \multirow{2}{*}{\textbf{Method}} & \multirow{2}{*}{\textbf{Backbone}} & 
% % \textbf{miniImageNet $\to$ CUB} \\ && 5-shot \\
% \hline
% MAML \tstrut & 52.70 $\pm$ 0.32\% & 55.52 $\pm$ 0.50\% & 55.82 $\pm$ 0.50\%\\
% %ANIL         & 55.82 $\pm$ 0.21\% & 52.70 $\pm$ 0.32\% & 52.70 $\pm$ 0.32\%\\
% ALFA         & 58.35 $\pm$ 0.25\% & 60.12 $\pm$ 0.49\% & 59.76 $\pm$ 0.49\%\\
% L2F          & 60.89 $\pm$ 0.22\% & 61.99 $\pm$ 0.49\% & 63.73 $\pm$ 0.48\%\\
% BOIL         & 60.84 $\pm$ 0.45\% & 52.46 $\pm$ 0.46\% & 63.28 $\pm$ 0.45\%\\
% CxGrad (Ours) \bstrut & \textbf{63.92 $\pm$ 0.44\%} & 53.75 $\pm$ 0.46\% & \textbf{64.85 $\pm$ 0.44\%}\\
% \hline
% %\end{tabular}
% \end{tabularx}
% \end{center}
% \caption{Test accuracy on 5-way 5-shot cross-domain few-shot classification.}
% \label{table:cross_domain}
% \end{table*}

% \begin{table}[t]
% %\fontsize{7}{10}\selectfont
% \begin{center}
% \begin{tabular}{c|c|c}
% %\begin{tabularx}{\textwidth}{>{\centering\arraybackslash}X|>{\centering\arraybackslash}X|>{\centering\arraybackslash}X|>{\centering\arraybackslash}X}
% \hline \hline
% \multirow{2}{*}{\textbf{Method}} \tstrut & \multicolumn{2}{c}{\textbf{miniImageNet}} \bstrut\\
% \cline{2-3}
% & \textbf{$\to$ CUB} & \textbf{$\to$ CIFAR-FS}\tstrut \bstrut\\
% %\tstrut & $\to$ CUB & $\to$ Omniglot & $\to$ FC100 & $\to$ CIFAR-FS \bstrut\\
% % \multirow{2}{*}{\textbf{Method}} & \multirow{2}{*}{\textbf{Backbone}} & 
% % \textbf{miniImageNet $\to$ CUB} \\ && 5-shot \\
% \hline
% MAML \tstrut & $52.70 \pm 0.32\%$ & $55.82 \pm 0.50\%$\\
% %ANIL         & 55.82 $\pm$ 0.21\% & 52.70 $\pm$ 0.32\% & 52.70 $\pm$ 0.32\%\\
% ALFA         & $58.35 \pm 0.25\%$ & $59.76 \pm 0.49\%$\\
% BOIL         & $60.84 \pm 0.45\%$ & $63.28 \pm 0.45\%$\\
% L2F          & $60.89 \pm 0.22\%$ & $63.73 \pm 0.48\%$\\
% CxGrad (Ours) \bstrut & \vcsb{63.92 \pm 0.44\%} & \vcsb{64.85 \pm 0.44\%}\\
% \hline
% \end{tabular}
% %\end{tabularx}
% \end{center}
% \caption{Test accuracy on 5-way 5-shot cross-domain few-shot classification.}
% \label{table:cross_domain}
% \end{table}

\begin{table}[t]
\setlength{\abovecaptionskip}{0pt}
\setlength{\belowcaptionskip}{-5pt}
%\fontsize{7}{10}\selectfont
\begin{center}
\begin{tabular}{@{}ccc@{}}
%\begin{tabularx}{\textwidth}{>{\centering\arraybackslash}X|>{\centering\arraybackslash}X|>{\centering\arraybackslash}X|>{\centering\arraybackslash}X}
\toprule %\toprule
\multirow{2}{*}{\textbf{Method}} & \multicolumn{2}{c}{\textbf{miniImageNet}} \\
%\cmidrule{2-3}
& \textbf{$\to$ CUB} & \textbf{$\to$ CIFAR-FS} \\
%\tstrut & $\to$ CUB & $\to$ Omniglot & $\to$ FC100 & $\to$ CIFAR-FS \bstrut\\
% \multirow{2}{*}{\textbf{Method}} & \multirow{2}{*}{\textbf{Backbone}} & 
% \textbf{miniImageNet $\to$ CUB} \\ && 5-shot \\
\midrule
MAML          & $52.70 \pm 0.32\%$ & $55.82 \pm 0.50\%$\\
%ANIL         & 55.82 $\pm$ 0.21\% & 52.70 $\pm$ 0.32\% & 52.70 $\pm$ 0.32\%\\
ALFA          & $58.35 \pm 0.25\%$ & $59.76 \pm 0.49\%$\\
BOIL          & $60.84 \pm 0.45\%$ & $63.28 \pm 0.45\%$\\
L2F           & $60.89 \pm 0.22\%$ & $63.73 \pm 0.48\%$\\
CxGrad (Ours) & \vcsb{63.92 \pm 0.44\%} & \vcsb{64.85 \pm 0.44\%}\\
\bottomrule
\end{tabular}
%\end{tabularx}
\end{center}
\caption{Test accuracy on 5-way 5-shot cross-domain few-shot classification on two meta-test datasets.}
\label{table:cross_domain}
\end{table}

==> WACV 2022 CxGrad/materials/table3_ablation_context_params_update_scheme.tex <==
% \begin{table}
% %\fontsize{9}{11}\selectfont
% \begin{center}
% \begin{tabular}{c|c}
% %\begin{tabularx}{\linewidth}{>{\centering\arraybackslash}X|>{\centering\arraybackslash}X}
% \hline \hline
% %Context vector & \multirow{2}{*}{CxGrad (Ours)}\\
% %learning rate  & \\
% \textbf{Context Parameter Update} & \textbf{Accuracy} \tstrut \bstrut \\
% \hline
% %step-wise & 68.83 $\pm$ 0.43\% \tstrut \\
% %task-wise & \bftab{69.91 $\pm$ 0.42\%} \bstrut\\
% step-wise & $68.83 \pm 0.43\%$ \tstrut \\
% %task-wise & \bm{$69.91 \pm 0.42\%$} \bstrut\\
% task-wise & \vcsb{69.82 \pm 0.42\%} \bstrut\\
% \hline
% \end{tabular}
% %\end{tabularx}
% \end{center}
% \caption{Ablation Studies on context parameter update scheme. The results are reported on 5-way 5-shot miniImageNet classification.}
% \label{table:ablation_update_scheme}
% \end{table}

\begin{table}[t]
\setlength{\abovecaptionskip}{0pt}
%\setlength{\belowcaptionskip}{-10pt}
%\fontsize{9}{11}\selectfont
\begin{center}
\begin{tabular}{cc}
%\begin{tabularx}{\linewidth}{>{\centering\arraybackslash}X|>{\centering\arraybackslash}X}
\toprule %\toprule
%Context vector & \multirow{2}{*}{CxGrad (Ours)}\\
%learning rate  & \\
\textbf{Update scheme for $\boldnu_{i}$} & \textbf{Accuracy}\\
\midrule
%step-wise & 68.83 $\pm$ 0.43\% \tstrut \\
%task-wise & \bftab{69.91 $\pm$ 0.42\%} \bstrut\\
step-wise & $68.83 \pm 0.43\%$\\
%task-wise & \bm{$69.91 \pm 0.42\%$} \bstrut\\
task-wise & \vcsb{69.82 \pm 0.42\%}\\
\bottomrule
\end{tabular}
%\end{tabularx}
\end{center}
\caption{Effect of context parameter update scheme. The accuracy results from 5-way 5-shot on miniImageNet.}
\label{table:ablation_update_scheme}
\end{table}

==> WACV 2022 CxGrad/materials/table4_ablation_step.tex <==
% \begin{table}[b]
% \fontsize{9}{11}\selectfont
% \begin{center}
% \begin{tabular}{c|c|c|c|c|c}
% \hline \hline
% %Context vector & \multirow{2}{*}{CxGrad (Ours)}\\
% %learning rate  & \\
% \multirow{3}{*}{\textbf{Accuracy}} \tstrut & \multicolumn{5}{c}{\textbf{inner-loop step}} \bstrut \\
% \cline{2-6}
% \tstrut & 1 & 2 & 3 & 4 & 5 \bstrut \\
% \cline{2-6}
%  & 69.12 \tstrut & 00.00 & 00.00 & 00.00 & \textbf{69.91} \bstrut\\
% \hline
% \end{tabular}
% \end{center}
% \caption{Ablation Studies on context parameter update scheme. The results are reported on 5-way 5-shot miniImageNet classification.}
% \label{table:num_steps}
% \end{table}

% \begin{table}[b]
% %\fontsize{9}{11}\selectfont
% \begin{center}
% \begin{tabular}{c|c|c|c|c|c}
% \hline \hline
% %Context vector & \multirow{2}{*}{CxGrad (Ours)}\\
% %learning rate  & \\
% %\multicolumn{5}{c}{\textbf{inner-loop step}} \tstrut \bstrut \\
% %\cline{1-5}
% \textbf{Step} \tstrut & \bf{1} & \textbf{2} & \textbf{3} & \textbf{4} & \textbf{5} \bstrut \\
% \hline
% %\cline{1-5}
% \textbf{Accuracy} \tstrut & $69.12$ & $69.33$ & $69.16$ & $69.53$ & \vcsb{69.82} \bstrut\\
% \hline
% \end{tabular}
% \end{center}
% \caption{Ablation Study on the effect of the number of inner-loop steps. The results are reported on 5-way 5-shot miniImageNet classification.}
% \label{table:ablation_num_steps}
% \end{table}

\begin{table}[t]
\setlength{\abovecaptionskip}{0pt}
% \setlength{\belowcaptionskip}{-5pt}
%\fontsize{9}{11}\selectfont
\begin{center}
\begin{tabular}{cccccc}
\toprule %\toprule
%Context vector & \multirow{2}{*}{CxGrad (Ours)}\\
%learning rate  & \\
%\multicolumn{5}{c}{\textbf{inner-loop step}} \tstrut \bstrut \\
%\cline{1-5}
\textbf{Step} & \textbf{1} & \textbf{2} & \textbf{3} & \textbf{4} & \textbf{5}\\
\midrule
%\cline{1-5}
\textbf{Accuracy} & $69.12$ & $69.33$ & $69.16$ & $69.53$ & \vcsb{69.82}\\
\bottomrule
\end{tabular}
\end{center}
%\caption{The effect of the number of inner-loop steps. The results are for 5-way 5-shot on miniImageNet.}
\caption{Ablation study on the number of inner-loop steps.}
\label{table:ablation_num_steps}
\end{table}

==> WACV 2022 CxGrad/materials/table5_ablation_context_lr.tex <==
% \begin{table}[t]
% \fontsize{9}{11}\selectfont
% \begin{center}
% \begin{tabular}{c|c|c}
% \hline \hline
% %Context vector & \multirow{2}{*}{CxGrad (Ours)}\\
% %learning rate  & \\
% \textbf{Setting} & \textbf{Context vector learning rate ($\beta$)} & \textbf{Accuracy} \tstrut \bstrut \\
% \hline
% \multirow{3}{*}{1-shot} \tstrut \bstrut & $0.01$ & $51.56$ \\
% & $0.1$ & $51.29$ \\
% & $1.0$ & \vcsb{51.80} \\
% \hline
% \multirow{3}{*}{5-shot} \tstrut \bstrut & $0.01$ & $69.28$\\
% & $0.1$ & $69.34$\\
% & $1.0$ & \vcsb{69.82}\\
% \hline
% \end{tabular}
% \end{center}
% \caption{Ablation Study on the various learning state for context parameter. The results are reported on 5-way 5-shot miniImageNet classification.}
%  \label{table:ablation_lr}
% \end{table}

\begin{table}[t]
\setlength{\abovecaptionskip}{0pt}
\setlength{\belowcaptionskip}{-13pt}
\fontsize{9}{11}\selectfont
\begin{center}
\begin{tabular}{ccc}
\toprule %\toprule
%Context vector & \multirow{2}{*}{CxGrad (Ours)}\\
%learning rate  & \\
%\textbf{Setting} 
& \textbf{Context parameter lr ($\beta$)} & \textbf{Accuracy}\\
\midrule
\multirow{3}{*}{1-shot} & $0.01$ & $51.56$ \\
& $0.1$ & $51.29$ \\
& $1.0$ & \vcsb{51.80} \\
\midrule
\multirow{3}{*}{5-shot} & $0.01$ & $69.28$\\
& $0.1$ & $69.34$\\
& $1.0$ & \vcsb{69.82}\\
\bottomrule
\end{tabular}
\end{center}
\caption{Ablation study on the learning rate for the context parameters.}
 \label{table:ablation_lr}
\end{table}

% \begin{table}[t]
% %\fontsize{9}{11}\selectfont
% \begin{center}
% \begin{tabular}{c|c}
% \hline \hline
% %Context vector & \multirow{2}{*}{CxGrad (Ours)}\\
% %learning rate  & \\
% \textbf{Context parameter learning rate ($\beta$)} & \textbf{Accuracy} \tstrut \bstrut \\
% % \hline
% % \multirow{3}{*}{1-shot} \tstrut \bstrut & 0.01 & 51.56 \\
% % & 0.1 & 51.29 \\
% % & 1.0 & \textbf{51.80} \\
% \hline
% 0.01 & 69.28\\
% 0.1 & 69.34\\
% 1.0 & \textbf{69.91}\\
% \hline
% \end{tabular}
% \end{center}
% \caption{Ablation Study on the various learning state for context parameter. The results are reported on 5-way 5-shot miniImageNet classification.}
% \label{table:ablation_lr}
% \end{table}

==> WACV 2022 CxGrad/materials/table6_resnet12_mini_imagenet.tex <==
\begin{table}[t]
\setlength{\abovecaptionskip}{0pt}
\setlength{\belowcaptionskip}{-5pt}
%\fontsize{7}{10}\selectfont
\begin{center}
\begin{tabular}{@{}ccc@{}}
\toprule
\multirow{2}{*}{\textbf{Method}} & \multicolumn{2}{c}{\textbf{miniImageNet}} \\
& \textbf{1-shot} & \textbf{5-shot} \\
\midrule
MAML~\cite{MAML} & $58.37 \pm 0.49\%$ & $69.76 \pm 0.46\%$\\
BOIL~\cite{BOIL} & - & $71.30 \pm 0.28\%$\\
L2F~\cite{L2F}   & $59.71 \pm 0.49\%$ & $77.04 \pm 0.42\%$\\
ALFA~\cite{ALFA} & $59.74 \pm 0.49\%$ & \vcsb{77.96 \pm 0.41\%}\\
CxGrad (Ours)    & \vcsb{60.19\pm0.45\%} & $75.17\pm0.40\%$\\
\bottomrule
\end{tabular}
%\end{tabularx}
\end{center}
\caption{Test accuracy on 5-way miniImageNet classification.}
\label{table:resnet12_mini_imagenet}
\end{table}

==> WACV 2022 CxGrad/materials/table7_resnet12_tiered_iamgenet.tex <==
\begin{table}[t]
\setlength{\abovecaptionskip}{0pt}
\setlength{\belowcaptionskip}{-5pt}
%\fontsize{7}{10}\selectfont
\begin{center}
\begin{tabular}{@{}ccc@{}}
\toprule
\multirow{2}{*}{\textbf{Method}} & \multicolumn{2}{c}{\textbf{tieredImageNet}} \\
& \textbf{1-shot} & \textbf{5-shot} \\
\midrule
MAML~\cite{MAML} & $58.58 \pm 0.49\%$  & $71.24 \pm 0.43\%$ \\
L2F~\cite{L2F}   & $64.04 \pm 0.48\%$  & $81.13 \pm 0.39\%$ \\
ALFA~\cite{ALFA} & $64.62 \pm 0.49\%$  & $82.48 \pm 0.38\%$ \\
CxGrad (Ours)    & \vcsb{65.47\pm0.44\%} & \vcsb{82.52\pm0.35\%} \\
\bottomrule
\end{tabular}
%\end{tabularx}
\end{center}
\caption{Test accuracy on 5-way tieredImageNet classification.}
\label{table:resnet12_tiered_imagenet}
\end{table}
